Spatio-Temporal Action Detection Under Large Motion

Current methods for spatiotemporal action tube detection often extend a bounding box proposal at a given keyframe into a 3D temporal cuboid and pool features from nearby frames. However, such pooling fails to accumulate meaningful spatiotemporal features if the position or shape of the actor shows large 2D motion and variability through the frames, due to large camera motion, large actor shape deformation, fast actor action and so on. In this work, we aim to study the performance of cuboid-aware feature aggregation in action detection under large action. Further, we propose to enhance actor feature representation under large motion by tracking actors and performing temporal feature aggregation along the respective tracks. We define the actor motion with intersection-over-union (IoU) between the boxes of action tubes/tracks at various fixed time scales. The action having a large motion would result in lower IoU over time, and slower actions would maintain higher IoU. We find that track-aware feature aggregation consistently achieves a large improvement in action detection performance, especially for actions under large motion compared to the cuboid-aware baseline. As a result, we also report state-of-the-art on the large-scale MultiSports dataset. The Code is available at https://github.com/gurkirt/ActionTrackDetectron.

==> configurations/packages.tex <==
\usepackage{graphicx}
\usepackage{svg}
\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{color}
\usepackage{ruler}
\usepackage{booktabs} % To thicken table lines
% \usepackage[colorlinks=false,hidelinks,nolinks=true]{hyperref}
\usepackage{caption}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{listings}
%  Sorts references in ascending order
\usepackage[numbers,sort]{natbib}
\usepackage[capitalize]{cleveref}
\newcommand{\colorRef}[1]{\textcolor{black}{#1}}
\crefname{figure}{\colorRef{Fig.}}{\colorRef{Figs.}}
\Crefname{figure}{\colorRef{Figure}}{\colorRef{Figures}}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{Tab.}{Tab.}{Tab.s}
\crefname{Tab.}{Tab.}{Tabs.}
\usepackage[inline]{enumitem}

==> figtex/FIG_large_visuals_two.tex <==
\begin{figure}[t] 
  \centering
  \includegraphics[width=.47\textwidth]{figures/large_motion_action_tworows.pdf}
  %\vskip 2mm
  \caption{
  %Ground-truth boxes and frames (dot at bottom of frame) annotated in green colour, detected track shown in red colour. 
  %Methods colour annotated in sub-captions with respective score colour on the bounding boxes of tracks.
  %Overlap, is spatio-temporal overlap of detected tube with ground-truth tube as defined by ~\cite{weinzaepfel2015learning}.
%   (a) TCN fail to detect it and others fail to detect initial few frames.
  (a) \lmotion due to fast action in Volley-spike instance detected with high overlap both by \aspp and \tcn and baseline fails to detect it. 
  Similarly, (b) \lmotion due to camera and baseline to detect and ASPP module shows better overlap than TCN.} 
%   \TODO{order of last subplot is reversed, need to fix to it. LUC: notice that I changed the caption.}}
  \label{fig:large_motion_visual} %\vspace{-3mm}
\end{figure}
